Prospects of measuring a metallicity trend and spread in globular clusters from low-resolution spectroscopy

The metallicity spread, or the metallicity trend along the evolutionary sequence of a globular cluster, is a rich source of information to help understand the cluster physics (e.g. multiple populations) and stellar physics (e.g. atomic diffusion). Low-resolution integral-field-unit spectroscopy in the optical with the MUSE is an attractive prospect if it can provide these diagnostics because it allows us to extract spectra of a large fraction of the cluster stars. We investigate the possibilities of full-spectrum fitting to derive stellar parameters and chemical abundances at low spectral resolution (R~2000). We reanalysed 1584 MUSE spectra of 1061 stars above the turn-off of NGC 6397 using FERRE and employing two different synthetic libraries. We derive the equivalent iron abundance \fehe for fixed values of \afe. We find that (i) the interpolation schema and grid mesh are not critical for the precision, metallicity spread, and trend; (ii) with the two grids, \fehe increases by ~0.2 dex along the sub-giant branch, starting from the turn-off of the main sequence; (iii) restricting the wavelength range to the optical decreases the precision significantly; and (iv) the precision obtained with the synthetic libraries is lower than the precision obtained previously with empirical libraries. Full-spectrum fitting provides reproducible results that are robust to the choice of the reference grid of synthetic spectra and to the details of the analysis. The \fehe increase along the sub-giant branch is in stark contrast with the nearly constant iron abundance previously found with empirical libraries. The precision of the measurements (0.05 dex on \fehe) is currently not sufficient to assess the intrinsic chemical abundance spreads, but this may change with deeper observations. Improvements of the synthetic spectra are still needed to deliver the full possibilities of full-spectrum fitting.

==> addbib <==
#!/bin/sh
## This small script retrieve a bibtex record from ADS passing a bibcode
## Philippe Prugniel 2008/01/08
## Example:
##  addbib mybib.bib 2004AJ....128...89D,ref1 2007ApJ...668..130C

usage="USAGE: addbib <bibtex_file> <bibcode>[,abrev] [<bibcode>[,abrev] ...]"

test $# -lt "2" && { echo $usage; exit 1; }

test -f $1 || { echo "this bibtex file does not exist ($1)"; exit 1; }
bibtex=$1

larg=$(echo $@ | sed "s/^[^ ]*\ //")   # list of arguments, after the first

for arg in $larg; do

multi=$(echo $arg | grep -c ',')

if test $multi -eq 0; then
  code=$(echo "$arg"|sed "s/&/%26/")
  echo "wget -q \"http://cdsads.u-strasbg.fr/cgi-bin/nph-abs_connect?data_type=BIBTEX&type=FILE&all=+Retrieve+record+&bibcodes=$code\" -O - >> $bibtex"
# change of ADS URLS on 2011/02/18
#  wget -q "http://cdsads.u-strasbg.fr/cgi-bin/nph-abs_connect?data_type=BIBTEX&type=FILE&all=+Retrieve+record+&bibcodes=$code" -O - | grep -v "^Retrieved 0 abstracts." >> $bibtex 
# Complete change at ADS 2019/11
#wget -q "http://cdsads.u-strasbg.fr/cgi-bin/nph-abs_connect?data_type=BIBTEX&all=+Retrieve+record+&bibcodes=$code" -O - |tail +6| grep -v "^Retrieved 0 abstracts." >> $bibtex
#  fortunately there is still an URL for this (do not have to use the API which require a spetial token)
# Note: the bibtex record is formatted in HTML ... we have to decode some entities:
#    &amp; -> &
#    &#34; -> "
#    &#39; -> '
  wget --quiet --no-check-certificate https://ui.adsabs.harvard.edu/abs/$code/exportcitation -O - | sed -n -e ':a' -e 'N' -e '$!ba' -e 's/.*<textarea[^>]*>\(.*\)>/\1/p' | sed -n -e ':a' -e 'N' -e '$!ba' -e 's/.<\/textarea>.*//p' | sed -e 's/\&amp;/\&/g' -e 's/\&#34;/"/g' -e "s/\&#39;/'/g" >> $bibtex

elif test $multi -eq 1; then
  read bibcode abrev << HERE
        $(IFS=,; echo $arg)
HERE
  duplic=$(grep -c "{$abrev," $bibtex)
  test $duplic -ne 0 && { echo "The abreviation ($abrev) already exists in ($bibtex) ... abort"; exit 1; }
  code=$(echo "$bibcode"|sed "s/&/%26/")
#  wget -q "http://cdsads.u-strasbg.fr/cgi-bin/nph-abs_connect?data_type=BIBTEX&type=FILE&all=+Retrieve+record+&bibcodes=$code" -O - | sed s/\{$bibcode,/\{$abrev,/ | grep -v "^Retrieved 0 abstracts.">> $bibtex
#  wget -q "http://cdsads.u-strasbg.fr/cgi-bin/nph-abs_connect?data_type=BIBTEX&all=+Retrieve+record+&bibcodes=$code" -O - |tail +6| sed s/\{$bibcode,/\{$abrev,/ | grep -v "^Retrieved 0 abstracts." >> $bibtex
  wget --quiet --no-check-certificate https://ui.adsabs.harvard.edu/abs/$code/exportcitation -O - | sed -n -e ':a' -e 'N' -e '$!ba' -e 's/.*<textarea[^>]*>\(.*\)>/\1/p' | sed -n -e ':a' -e 'N' -e '$!ba' -e 's/.<\/textarea>.*//p' | sed -e 's/\&amp;/\&/g' -e 's/\&#34;/"/g' -e "s/\&#39;/'/g" | sed s/\{$bibcode,/\{$abrev,/ >> $bibtex

else
  echo $usage
  exit 1
fi

done
exit

fi
## ---- end ------------------------------------------------------------------


==> makefile <==
# Latex Makefile: compile, clean
# 
# to produce a pdf file:         $ make
# to clean :		         $ make clean
# to test the compilation:       $ make test
# to process and display on mac: $ make mac
#
# MK 2009/15/14; revised PhP 2009/11/28; extended version for MUSEFERRE, PhP 2020/01/29

PAPER = paper#  # paper.tex, on the git

all: ${PAPER}.pdf

############################################################################################
# Targets for making the pdf of the paper 

# dependencies
BIB=paper.bib  # bibtex file managed on the git
#    figs/*, figures, for the moment on the git, but we will make them in the present makefile
FIGA1 = figs/ch2_map_linear_interp_ngc6397id000009229jd2456865p5898f000.pdf figs/ch2_map_linear_interp_stacked.pdf
FIG1 = figs/Fig1.pdf
FIGS2 = figs/Whole_range/Fig2a_Hbet_GSL.pdf \
       figs/Whole_range/Fig2a_Hbet_AP.pdf \
       figs/Whole_range/Fig2b_Mg_GSL.pdf \
       figs/Whole_range/Fig2b_Mg_AP.pdf \
       figs/Whole_range/Fig2b_Ca_GSL.pdf \
       figs/Whole_range/Fig2b_Ca_AP.pdf
FIG3 = figs/Whole_range/Fig3a_Teff.pdf figs/Whole_range/Fig3b_feh.pdf
FIG4 = figs/Whole_range/Fig4_Teff_FeH_GSL.pdf
FIG5 = figs/Whole_range/Fig5_compa_GSL_AP.pdf
FIG6 = figs/Whole_range/Fig6_normalisation.pdf
FIG8 = figs/Fig8_GSL_AP.pdf

FIG9 = figs/Different_ranges.pdf
FIG10 = figs/Different_ranges_AP.pdf
FIG11 = figs/Whole_range/Fig6a_comparison_Teff_solEnh.pdf figs/Whole_range/Fig6b_comaprison_feh_solEnh.pdf
FIGS=figs/* ${FIGA1} ${FIG1} ${FIGS2} ${FIG3} ${FIG4} ${FIG5} ${FIG6} ${FIG8} ${FIG9} ${FIG10} ${FIG11} 


TABL2=table_spread.tex
TABL3=table3_spread.tex
TABLS=${TABL2} ${TABL3}

STAT = figs/Whole_range/Fig_lsf_matching.pdf figs/Whole_range/Fig_wave_matching.pdf #  (procedure only for computing stats)

test: 
	pdflatex -halt-on-error -draftmode ${PAPER} || { exit 1; }

${PAPER}.pdf:  ${PAPER}.tex ${BIB} ${FIGS} ${TABLS}
	pdflatex -halt-on-error -draftmode ${PAPER} || { exit 1; }
	bibtex ${PAPER}; pdflatex ${PAPER}; pdflatex ${PAPER} 
	@make gitstat

mac: ${PAPER}.pdf gitstat;
	@open ${PAPER}.pdf

gitstat:
	@test `git status -s | grep -vc -e '^[?]'` -eq 0 || \
	{ echo 'There are un-committed files (do git commit?):'; git status -s | grep -v -e '^[?]'; }
	@git status | grep '^Your branch is ahead' && echo "Do 'git push'" || exit 0

clean: ${PAPER}.pdf
	rm *.aux *.log *.dvi *.out *.llt

############################################################################################
# Targets for making the figures and tables (tex and CDS) 
#
# Dependencies:
#    - measurements tables (results of FERRE, measurements from H16 and J20 stored on the git)
#    - spectra (for the figures showing fit examples)
#    - scripts and utilities
#   H16 catalogue of measurements 
MEAS_HUSSER = ../analysis/Plot_routines/file_dependencies/Husser_1587.txt
#   measurement with GSL (txt and mdl files are not available)
#MEAS_GSL = ../analysis/Results/GSL/whole_lambda_ncont60/inter3/parameters_cont3_inter3_gsl_interpol_lsf_ncgauss_full_lambda_afe0p4_wcs4750.opf \
#           ../analysis/Results/GSL/whole_lambda_ncont60/inter3/input_norm_cont3_inter3_gsl_interpol_lsf_ncgauss_full_lambda_afe0p4_wcs4750.txt \
#           ../analysis/Results/GSL/whole_lambda_ncont60/inter3/cont3_inter3_gsl_interpol_lsf_ncgauss_full_lambda_afe0p4_wcs4750.mdl
# two of the MEAS_GSL files are not on the git ... and for the moment it is not possible to make the figures
MEAS_GSL = ../analysis/Results/GSL/GSL_pix3680_afe0d4_i3_n3_d60_1.opf 
#   ??? (files not avalable on the git, are they needed?)
SPECTRA = ../analysis/Spectra/spectra_WHOLE_telluric_corrd.frd ../Spectra/Wfile_WHOLE.wav

UTIL = ../analysis/Plot_routines/figstyle.py ../analysis/Plot_routines/utilities.py

# Yet no target for Fig1 !!!!!!!!!!!

fig1: ${FIG1}; open $?  # on a mac, it make the fig and open with preview (have to make it portable)
${FIG1}: ../analysis/Plot_routines/Fig1.py ${UTIL} ../analysis/Plot_routines/file_dependencies/Husser16.txt 
	@cd ../analysis/Plot_routines/; python3 Fig1.py

figs2: ${FIGS2}; open $?
${FIGS2}: ../analysis/Plot_routines/Fig2.py ${UTIL} ../analysis/ferre/ngc6397id000010747jd2456866p4985f000_BF_model_AP.fits ../analysis/ferre/ngc6397id000010747jd2456866p4985f000_norm_AP_MUSE.fits ../analysis/ferre/ngc6397id000010747jd2456866p4985f000_BF_model_GSL.fits ../analysis/ferre/ngc6397id000010747jd2456866p4985f000_norm_GSL_MUSE.fits ../analysis/ferre/ngc6397id000010747jd2456866p4985f000_BF_model_AP_afeSOL.fits ../analysis/ferre/ngc6397id000010747jd2456866p4985f000_norm_AP_MUSE_afeSOL.fits ../analysis/ferre/ngc6397id000010747jd2456866p4985f000_BF_model_GSL_afeSOL.fits ../analysis/ferre/ngc6397id000010747jd2456866p4985f000_norm_GSL_MUSE_afeSOL.fits
	@cd ../analysis/Plot_routines/; python3 Fig2.py


fig3: ${FIG3}; open $?  # on a mac, it make the fig and open with preview (have to make it portable)
${FIG3}: ../analysis/Plot_routines/Fig3.py ${UTIL} ${MEAS_HUSSER} ../analysis/Results/GSL/GSL_pix3680_afe0d4_i3_n3_d60_1.opf
	@cd ../analysis/Plot_routines/; python3 Fig3.py

fig4: ${FIG4}; open $?
${FIG4}: ../analysis/Plot_routines/Fig4.py ${UTIL} ${MEAS_HUSSER} ../analysis/Results/GSL/GSL_pix3680_afe0d4_i1_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d4_i2_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d4_i3_n3_d60_1.opf 
	@cd ../analysis/Plot_routines/; python3 Fig4.py

fig5: ${FIG5}; open $?  
${FIG5}: ../analysis/Plot_routines/Fig5.py ${UTIL} ../analysis/Results/GSL/GSL_pix3680_afe0d4_i3_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix3680_afe0d5_i3_n3_d60_1.opf
	@cd ../analysis/Plot_routines/; python3 Fig5.py

fig6: ${FIG6}; open $?
${FIG6}: ../analysis/Plot_routines/Fig6.py ${UTIL} ../analysis/Results/GSL/GSL_pix3680_afe0d4_i3_n3_d30_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d4_i3_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d4_i3_n3_d120_1.opf
	@cd ../analysis/Plot_routines/; python3 Fig6.py

fig8: ${FIG8}; open $?
${FIG8}: ../analysis/Plot_routines/Fig8.py ${UTIL} ../analysis/Results/GSL/GSL_pix3680_afe0d4_i3_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix3680_afe0d5_i3_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix3680_afe0d5_i1_n3_d60_1.opf
	@cd ../analysis/Plot_routines/; python3 Fig8.py

#----------------------- 

fig9: ${FIG9}; open $?  
${FIG9}: ../analysis/Plot_routines/Fig9.py ${UTIL} ../analysis/Results/GSL/GSL_pix3680_afe0d4_i3_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix1641_afe0d4_i3_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix841_afe0d4_i3_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix2121_afe0d4_i3_n3_d60_1.opf
	@cd ../analysis/Plot_routines/; python3 Fig9.py

fig10: ${FIG10}; open $?
${FIG10}: ../analysis/Plot_routines/Fig10.py ${UTIL} ../analysis/Results/AP-FINE/AP_pix3680_afe0d5_i3_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix2121_afe0d5_i3_n3_d60_1.opf  ../analysis/Results/AP-FINE/AP_pix1641_afe0d5_i3_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix841_afe0d5_i3_n3_d60_1.opf
	@cd ../analysis/Plot_routines/; python3 Fig10.py

fig11: ${FIG11}; open $?  
${FIG11}: ../analysis/Plot_routines/Fig11.py ${UTIL} ../analysis/Results/GSL/GSL_pix3680_afe0d0_i3_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d4_i3_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix3680_afe0_i3_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix3680_afe0d5_i3_n3_d60_1.opf
	@cd ../analysis/Plot_routines/; python3 Fig11.py

lsf stat: ; @cd ../analysis/Plot_routines/; python3 Fig_mismatch.py

figvturb: ${FIGVTURM}; open $?
${FIGVTURB}: ../analysis/Plot_routines/Fig_vturb.py ${UTIL} ../analysis/Results/AP-FINE/AP_pix3680_v2_afe0d5_i3_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix3680_afe0d5_i3_n3_d60_1.opf 
	@cd ../analysis/Plot_routines/; python3 Fig_vturb.py

${TABL2}: ../analysis/Plot_routines/Table.py ${UTIL} ${MEAS_HUSSER} ../analysis/Results/GSL/GSL_pix3680_afe0d4_i1_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d4_i2_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d4_i3_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix1641_afe0d4_i3_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix1641_afe0d4_i2_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix1641_afe0d4_i1_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix841_afe0d4_i3_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix841_afe0d4_i2_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix841_afe0d4_i1_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix2121_afe0d4_i3_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix2121_afe0d4_i1_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix2121_afe0d4_i2_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d0_i1_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d0_i2_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d0_i3_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix1641_afe0d0_i3_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix1641_afe0d0_i2_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix1641_afe0d0_i1_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix841_afe0d0_i3_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix841_afe0d0_i2_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix841_afe0d0_i1_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix2121_afe0d0_i3_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix2121_afe0d0_i1_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix2121_afe0d0_i2_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix3680_afe0d5_i1_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix3680_afe0d5_i2_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix3680_afe0d5_i3_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix2121_afe0d5_i1_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix2121_afe0d5_i2_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix2121_afe0d5_i3_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix1641_afe0d5_i1_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix1641_afe0d5_i2_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix1641_afe0d5_i3_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix841_afe0d5_i1_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix841_afe0d5_i2_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix841_afe0d5_i3_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix3680_afe0_i1_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix3680_afe0_i2_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix3680_afe0_i3_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix2121_afe0_i1_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix2121_afe0_i2_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix2121_afe0_i3_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix841_afe0_i1_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix841_afe0_i2_n3_d60_1.opf ../analysis/Results/AP-FINE/AP_pix841_afe0_i3_n3_d60_1.opf ../analysis/Results/AP-COARSE/APC_pix3680_afe0d5_i1_n3_d60_1.opf ../analysis/Results/AP-COARSE/APC_pix3680_afe0d5_i2_n3_d60_1.opf ../analysis/Results/AP-COARSE/APC_pix3680_afe0d5_i3_n3_d60_1.opf
	@cd ../analysis/Plot_routines/; python3 Table.py

${TABL3}: ../analysis/Plot_routines/Table3.py ${UTIL} ../analysis/Results/GSL/GSL_pix3680_afe0d4_i1_n3_d30_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d4_i2_n3_d30_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d4_i3_n3_d30_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d4_i1_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d4_i2_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d4_i3_n3_d60_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d4_i1_n3_d120_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d4_i2_n3_d120_1.opf ../analysis/Results/GSL/GSL_pix3680_afe0d4_i3_n3_d120_1.opf
	@cd ../analysis/Plot_routines/; python3 Table3.py



############################################################################################
# Targets for making the FERRE measurements files
#  Dependencies:
#    - data files: observations and grids (stored locally, maybe later we will include targets for generating them)
#    - Command files for FERRE

FERRE_EXE=../analysis/ferre/src/a.out # path to the FERRE executable (every user must install FERRE there, or make a symlink)

# diagnostise the presence of FERRE, it may be executed as "make ferre"
ferre FERRE_EXE:
	@test -e ${FERRE_EXE} || { echo "Error, no FERRE executable at the expected location: ${FERRE_EXE}"; exit 1; }

# I do not know how it is presently organised:
#   - do you run directly FERRE, or do you have a script that massage the input, run FERRE, and massage the output?
#   - to make an example, I will here run FERRE on a simple example
#        The control file is input.nml, the model file: pfile, and the observations: ffile

# there is an example in FERRE:
#    control file =  input.nml_interpol
#    
FERRE_TEST_DIR=../analysis/philippe/ferre/test
ferre_test interpol.mdl: ${FERRE_EXE} ${FERRE_TEST_DIR}/input.nml_interpol ${FERRE_TEST_DIR}/interpol.ipf ${FERRE_TEST_DIR}/f_ki13_1000.dat
	@cp ${FERRE_TEST_DIR}/input.nml_interpol input.nml; \
	cp ${FERRE_TEST_DIR}/interpol.ipf .; \
	cp ${FERRE_TEST_DIR}/f_ki13_1000.dat .; \
	${FERRE_EXE} > interpol.log || { echo "Error, FERRE execution failed"; exit 1; }

# I suppose that the best is to have a FERRE directory where we store all the nml and the other input files, and were are generated the output files

# --- end ---


==> table3_spread.tex <==
% Metallicity spread for different normalisation windows, MUSEFERRE
% generated automatically by the procedure Table3.py: 2021-11-02 15:31:36.797812
% -----------------------------------------------------------------
\multirow{3}{*}{30}
& L & -1.950 & 0.084\\
& Q & -1.926 & 0.087\\
& C & -1.930 & 0.085\\

\hline
\multirow{3}{*}{60}
& L & -1.966 & 0.081\\
& Q & -1.942 & 0.084\\
& C & -1.945 & 0.082\\

\hline
\multirow{3}{*}{120}
& L & -1.934 & 0.086\\
& Q & -1.907 & 0.088\\
& C & -1.911 & 0.089\\
% ------- end of table --------------------------------------------


==> table_spread.tex <==
% Metallicity spread, MUSEFERRE
% generated automatically by the procedure Table.py: 2022-02-08 20:21:37.859856
% -----------------------------------------------------------------
GSL& 0 & $475 - 930$ & C & $-1.995$ &46& 0.080&  0.103&  $0.21$ \\
\midrule
\multicolumn{9}{c}{\cite{jain20}}\\
MIL& SN & $475 - 740$ & P & $-2.086$ &56& 0.078&  0.095&  $-0.05$ \\
\midrule\midrule

\multirow{3}{*}{GSL}& \multirow{3}{*}{$0.4$} & \multirow{3}{*}{$475 - 930$} & L & $-1.966$ &41& 0.060&  0.081&  $0.15$ \\
&  &  & Q & $-1.942$ &40& 0.063&  0.084&  $0.17$ \\
&  &  & C & $-1.945$ &41& 0.059&  0.082&  $0.18$ \\

\hline
\multirow{3}{*}{GSL}& \multirow{3}{*}{$0.4$} & \multirow{3}{*}{$475 - 740$} & L & $-2.186$ &50& 0.131&  0.137&  $0.28$ \\
&  &  & Q & $-2.180$ &50& 0.134&  0.142&  $0.28$ \\
&  &  & C & $-2.167$ &51& 0.133&  0.139&  $0.25$ \\

\hline
%\multirow{3}{*}{GSL}& \multirow{3}{*}{$0.4$} & \multirow{3}{*}{$475 - 680$} & L & $-2.183$ &50& 0.135&  0.140&  $0.28$ \\
%&  &  & Q & $-2.178$ &50& 0.137&  0.144&  $0.28$ \\
%&  &  & C & $-2.166$ &51& 0.136&  0.141&  $0.25$ \\

%\hline
\multirow{3}{*}{GSL}& \multirow{3}{*}{$0.4$} & \multirow{3}{*}{$475 - 580$} & L & $-2.224$ &56& 0.146&  0.159&  $0.33$ \\
&  &  & Q & $-2.218$ &55& 0.147&  0.164&  $0.33$ \\
&  &  & C & $-2.203$ &57& 0.149&  0.165&  $0.31$ \\

\midrule\midrule

\multirow{3}{*}{GSL}& \multirow{3}{*}{$0$} & \multirow{3}{*}{$475 - 930$} & L & $-1.727$ &42& 0.063&  0.086&  $0.19$ \\
&  &  & Q & $-1.704$ &42& 0.061&  0.082&  $0.16$ \\
&  &  & C & $-1.712$ &42& 0.061&  0.082&  $0.16$ \\

\hline
\multirow{3}{*}{GSL}& \multirow{3}{*}{$0$} & \multirow{3}{*}{$475 - 740$} & L & $-2.066$ &48& 0.130&  0.135&  $0.22$ \\
&  &  & Q & $-2.055$ &48& 0.133&  0.143&  $0.23$ \\
&  &  & C & $-2.047$ &48& 0.125&  0.131&  $0.21$ \\

\hline
%\multirow{3}{*}{GSL}& \multirow{3}{*}{$0$} & \multirow{3}{*}{$475 - 680$} & L & $-2.066$ &48& 0.132&  0.136&  $0.22$ \\
%&  &  & Q & $-2.054$ &48& 0.135&  0.143&  $0.23$ \\
%&  &  & C & $-2.048$ &48& 0.127&  0.132&  $0.21$ \\

%\hline
\multirow{3}{*}{GSL}& \multirow{3}{*}{$0$} & \multirow{3}{*}{$475 - 580$} & L & $-2.129$ &56& 0.151&  0.168&  $0.34$ \\
&  &  & Q & $-2.123$ &56& 0.154&  0.174&  $0.34$ \\
&  &  & C & $-2.109$ &56& 0.154&  0.171&  $0.33$ \\

\midrule\midrule

\multirow{3}{*}{\AP}& \multirow{3}{*}{$0.5$} & \multirow{3}{*}{$475 - 930$} & L & $-2.031$ &41& 0.055&  0.079&  $0.20$ \\
&  &  & Q & $-2.015$ &40& 0.052&  0.075&  $0.21$ \\
&  &  & C & $-2.014$ &41& 0.052&  0.075&  $0.21$ \\

\hline
\multirow{3}{*}{\AP}& \multirow{3}{*}{$0.5$} & \multirow{3}{*}{$475 - 740$} & L & $-1.945$ &48& 0.086&  0.113&  $0.46$ \\
&  &  & Q & $-1.928$ &47& 0.086&  0.112&  $0.46$ \\
&  &  & C & $-1.925$ &47& 0.084&  0.111&  $0.46$ \\

\hline
%\multirow{3}{*}{\AP}& \multirow{3}{*}{$0.5$} & \multirow{3}{*}{$475 - 680$} & L & $-1.941$ &49& 0.090&  0.116&  $0.46$ \\
%&  &  & Q & $-1.923$ &47& 0.089&  0.114&  $0.46$ \\
%&  &  & C & $-1.920$ &47& 0.087&  0.113&  $0.46$ \\

%\hline
\multirow{3}{*}{\AP}& \multirow{3}{*}{$0.5$} & \multirow{3}{*}{$475 - 580$} & L & $-2.092$ &61& 0.129&  0.137&  $0.39$ \\
&  &  & Q & $-2.074$ &62& 0.128&  0.134&  $0.40$ \\
&  &  & C & $-2.073$ &62& 0.127&  0.134&  $0.41$ \\

\midrule\midrule

\multirow{3}{*}{\AP}& \multirow{3}{*}{$0$} & \multirow{3}{*}{$475 - 930$} & L & $-1.650$ &42& 0.058&  0.081&  $0.24$ \\
&  &  & Q & $-1.636$ &41& 0.056&  0.079&  $0.25$ \\
&  &  & C & $-1.635$ &42& 0.056&  0.079&  $0.25$ \\

\hline
\multirow{3}{*}{\AP}& \multirow{3}{*}{$0$} & \multirow{3}{*}{$475 - 740$} & L & $-1.758$ &50& 0.089&  0.120&  $0.47$ \\
&  &  & Q & $-1.744$ &50& 0.091&  0.122&  $0.47$ \\
&  &  & C & $-1.741$ &50& 0.091&  0.121&  $0.47$ \\

\hline
\multirow{3}{*}{\AP}& \multirow{3}{*}{$0$} & \multirow{3}{*}{$475 - 580$} & L & $-1.925$ &62& 0.145&  0.148&  $0.42$ \\
&  &  & Q & $-1.908$ &63& 0.143&  0.147&  $0.44$ \\
&  &  & C & $-1.907$ &63& 0.143&  0.146&  $0.45$ \\

\midrule\midrule

\multirow{3}{*}{APC}& \multirow{3}{*}{$0.5$} & \multirow{3}{*}{$475 - 930$} & L & $-2.068$ &42& 0.061&  0.083&  $0.20$ \\
&  &  & Q & $-2.023$ &41& 0.055&  0.077&  $0.20$ \\
&  &  & C & $-2.013$ &40& 0.051&  0.074&  $0.22$ \\
% ------- end of table --------------------------------------------

